Multiparticle Kalman filter for object localization in symmetric environments

This study considers the object localization problem and proposes a novel multiparticle Kalman filter to solve it in complex and symmetric environments. Two well-known classes of filtering algorithms to solve the localization problem are Kalman filter-based methods and particle filter-based methods. We consider these classes, demonstrate their complementary properties, and propose a novel filtering algorithm that takes the best from two classes. We evaluate the multiparticle Kalman filter in symmetric and noisy environments. Such environments are especially challenging for both classes of classical methods. We compare the proposed approach with the particle filter since only this method is feasible if the initial state is unknown. In the considered challenging environments, our method outperforms the particle filter in terms of both localization error and runtime.

==> 43_KPF_discussion.tex <==
\section{Kalman and particle filters discussion}


Table~\ref{tab::kf_vs_pf} presents the overview of the main equations of Kalman and particle filters~\cite{kf_overview}.
We highlight the complementary properties of these methods that motivate us to develop a novel method that will take the best from Kalman and particle filters.

\begin{table}[!ht]
    \centering
    \caption{Kalman and particle filter equations}
    \begin{tabular}{ c c c}
\toprule
Stage & Extended Kalman filter & Particle filter\\
\midrule
 Predict                            &  
 $\rvx_{t+1}^- = f(\rvx_t, \rvu_t)$                  &
 $\rvx_{t+1}^i = f(\rvx_t^i, \rvu_t, \eta^i)$       \\
                                       &
$\mP_{t+1}^- = \mF \mP_{t} \mF^T + \mQ_{t+1}$    &
                                      \\
& $\mF = \left.\frac{\partial f(\rvx, \rvu_{t+1})}{\partial \rvx}\right|_{\rvx = \rvx_t}$                           \\                                      
                                      \midrule
 Update                           &
 $\rvz_{t+1} = g(\rvx_{t+1}^-)$              &
 $\rvz_{t+1}^i = g(\rvx_{t+1}^i) + \zeta^i$  \\
                                       &
$\mH_{t+1} = \frac{\partial g(\rvx)}{\partial \rvx}|_{\rvx = \rvx^-_{t+1}}$                    &
$w_{t+1}^i\sim w_t^i p(\rvz_{t+1}^i|\rvx_{t+1}^i)$
                                       \\
                                       &
$\mS = \mH_{t+1} \mP_{t+1}^- \mH_{t+1}^T + \mR$        &
$i_1..i_N \sim Multinomial(w^1_{t+1}..w^N_{t+1})$                   \\
     &
$\mK_{t+1} = \mP_{t+1}^- \mH_{t+1}^T \mS^{-1}$ & 
$\rvx^1_{t+1}..\rvx^N_{t+1} \leftarrow  \rvx^{i_1}_{t+1}..\rvx^{i_N}_{t+1}$                \\
                                       &
$\rvx_{t+1} = \rvx_{t+1}^- + \mK_{t+1} (\rvz_{t+1} - \tilde{\rvz}_{t+1}^i)$ 
                                       &
$w^i_t=\frac{1}{N}$              \\
                                       &
$\mP_{t+1} = (\mI - \mK_{t+1} \mH_{t+1})\mP_{t+1}^-$
                                       &
                                       \\
\bottomrule
\end{tabular}
\label{tab::kf_vs_pf}
\end{table}



% Kalman filter is much faster and requires less memory than the particle filter.
% However, it has strict assumptions like Gaussian noise assumption, initial state knowledge, etc.
% It causes its popularity despite the constraints such as Gaussian noise assumption, initial state knowledge, etc. 
% multiple modifications try to extend the Kalman filter to the broader class of problems. 
% At the same time, particle filters are very popular due to their simplicity, increasing power of modern computers, and the opportunity to perform parallel computations.


